Interpretable Affordance Detection on 3D Point Clouds with Probabilistic Prototypes

Robotic agents need to understand how to interact with objects in their environment, both autonomously and during human-robot interactions. Affordance detection on 3D point clouds, which identifies object regions that allow specific interactions, has traditionally relied on deep learning models like PointNet++, DGCNN, or PointTransformerV3. However, these models operate as black boxes, offering no insight into their decision-making processes. Prototypical Learning methods, such as ProtoPNet, provide an interpretable alternative to black-box models by employing a "this looks like that" case-based reasoning approach. However, they have been primarily applied to image-based tasks. In this work, we apply prototypical learning to models for affordance detection on 3D point clouds. Experiments on the 3D-AffordanceNet benchmark dataset show that prototypical models achieve competitive performance with state-of-the-art black-box models and offer inherent interpretability. This makes prototypical models a promising candidate for human-robot interaction scenarios that require increased trust and safety.

==> tab/multi_label_pointnet.tex <==
\begin{table}[tb]
\centering
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{12pt}
\caption{Affordance Detection metrics of PointNet++ and the prototypical model with PointNet++ backbone on the 3D AffordanceNet validation dataset with multi-label annotations.}
\label{tab:average_res_label}
\begin{tabular}{@{}lcc@{}}
\toprule
\multirow{2}{*}{\textbf{Metrics}} & \multicolumn{2}{c}{\textbf{Multi-Label Experiment}} \\
\cmidrule(lr){2-3}
& \textbf{PointNet++} & \textbf{Prototypical Model} \\ 
\midrule
mIoU & 14.9 & \textbf{17.9} \\
mAP & 41.8 & \textbf{47.1} \\
mAUC & 84.8 & \textbf{86.8} \\
MSE $\downarrow$ & 0.040 & \textbf{0.030} \\
\bottomrule
\end{tabular}
\end{table}
